Causal Discovery over High-Dimensional Structured Hypothesis Spaces with Causal Graph Partitioning

The aim in many sciences is to understand the mechanisms that underlie the observed distribution of variables, starting from a set of initial hypotheses. Causal discovery allows us to infer mechanisms as sets of cause and effect relationships in a generalized way -- without necessarily tailoring to a specific domain. Causal discovery algorithms search over a structured hypothesis space, defined by the set of directed acyclic graphs, to find the graph that best explains the data. For high-dimensional problems, however, this search becomes intractable and scalable algorithms for causal discovery are needed to bridge the gap. In this paper, we define a novel causal graph partition that allows for divide-and-conquer causal discovery with theoretical guarantees. We leverage the idea of a superstructure -- a set of learned or existing candidate hypotheses -- to partition the search space. We prove under certain assumptions that learning with a causal graph partition always yields the Markov Equivalence Class of the true causal graph. We show our algorithm achieves comparable accuracy and a faster time to solution for biologically-tuned synthetic networks and networks up to ${10^4}$ variables. This makes our method applicable to gene regulatory network inference and other domains with high-dimensional structured hypothesis spaces.

==> figs/tex/exp2.tex <==
\begin{figure}[t]
    \centering
    % \includegraphics[width=0.9\linewidth]{figs/experiments/fig_exp2.png}
    \includegraphics[width=\linewidth]{figs/plots/prob_interedge/TPR_multi_algs.pdf}
    \caption{Experiment increasing number of edges between communities. }
    \label{fig:exp_2}
\end{figure}

==> figs/tex/exp5.tex <==
\begin{figure}[t]
    % \includegraphics[width=0.9\linewidth]{figs/experiments/time_exp5.png}
    % \includegraphics[width=\linewidth]{figs/plots/num_nodes/timing.pdf}
    \centering
    \includegraphics[width=0.95\linewidth]{figs/plots/num_nodes/fixed-timing.pdf}
    \caption{ 
        Hierarchical graphs with increasing number of nodes from 10 to 10,000. 
        This experiment was run with a 2.8~GHz 
        % AMD EPYC Milan 7543P 
        64 core CPU with 512~GB of DDR4 RAM.  
    }
    \label{fig:experiment_5}
\end{figure}

==> figs/tex/exps1-2.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.85\linewidth]{figs/plots/subplots/exps1-2.pdf}
    \caption{
        \ul{Left Column}: 
        Experiment increasing the \# of samples $\bm{n}$. Error bars are $\bm{95\%}$ confidence intervals.
        \ul{Right Column}: 
        Experiment increasing \# of edges between communities.
    }
    \label{fig:exp_1_2}
\end{figure}

==> figs/tex/exps3-4.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.85\linewidth]{figs/plots/subplots/exps3-4.pdf}
    \caption{
        \ul{Left Column}: 
         Experiment increasing fraction of extraneous edges in a perfect superstructure.
        %
        \ul{Right Column}: 
        Increase in density of the imperfect superstructure by increasing the significant level $\bm{\alpha}$ of the PC algorithm.
    }
    \label{fig:exp_3_4}
\end{figure}

==> pseudocode/1_screen.tex <==
\begin{algorithm}[t]
\small
\KwIn{a superstructure $G$, a set of mixed graphs $G_i = (S_i, E_i)$ for $E_i$ containing directed and bidirected edges, a boolean flag $\texttt{take\_subset}$ with default value \texttt{True}}
\KwResult{$G_{\text{out}} = (V^*,E^*)$ a directed graph}

    \ForEach{$i=1,\ldots,N$}{
        \tcp{Ignore bidirected edges.}
        $E_{\text{candidates}} \gets E_{\text{candidates}}\cup \left\{(u,v) \in E_i\right\}$\; 
        \label{line:discard_bidirected_and_not_in_ss}
    }

    \If{\texttt{take\_subset}}{
        \tcp{Discard edges not in superstructure.}
        $E_{\text{candidates}} \gets E_{\text{candidates}} \cap \text{edges}(G)$\;
    }
    
    \ForEach{$(u,v) \in E_{\text{candidates}}$}{
        \If{$(u,v)\in E_j \ \forall j$ s.t. $S_j \supseteq \{u,v\}$}{
            \tcp{If an edge $(u,v)$ appears in the learned output on all subsets that contain both $u$ and $v$, add edge to output graph.}
            $E^* \gets E^{*} \cup \{(u,v)\}$\;
            \label{line:favor_no_edge}
        }
    }

    \Return $G_{\text{out}} = (V^*,E^*)$\;

\caption{\screenprojections{}}
\label{alg:screening}
\end{algorithm}

% \begin{algorithm}[t]
% \caption{\screenprojections$(G, \left\{G_i = (S_i, E_i)\right\}_{i=1}^N, \texttt{take\_subset} = \texttt{True})$}\label{alg:screening}
% \begin{algorithmic}
% \REQUIRE a superstructure $G$, a set of mixed graphs $G_i = (S_i, E_i)$ for $E_i$ containing directed and bidirected edges, a boolean flag $\texttt{take\_subset}$ with default value \texttt{True}.
% \ENSURE $G_{\text{out}} = (V^*,E^*)$ a directed graph
% \STATE $V^* \gets \bigcup_{i=1}^N S_i$ \COMMENT{Initialize global node set}
% \STATE $E^* \gets \emptyset$ \COMMENT{Initialize empty edge set}
% \STATE $E_{\text{candidates}} \gets \emptyset$

% \FOR{$i=1,\dots,N$}
%     \STATE $E_{\text{candidates}} \gets E_{\text{candidates}}\cup \left\{(u,v) \in E_i\right\}$ \COMMENT{Ignore bidirected edges.}\label{line:discard_bidirected_and_not_in_ss}
% \ENDFOR\\
% \IF{\texttt{take\_subset}}
%     \STATE $E_{\text{candidates}} \gets E_{\text{candidates}}\cap \text{edges}(G)$ \COMMENT{Discard edges not in superstructure.}
% \ENDIF
% \FOR{$(u,v) \in E_{\text{candidates}}$}
%     \IF{$(u,v)\in E_j \ \forall j$ s.t. $S_j \supseteq \{u,v\}$}
%             \STATE $E^* \gets E^{*} \cup \{(u,v)\}$ \COMMENT{If an edge $(u,v)$ appears in the learned output on all subsets that contain both $u$ and $v$, add edge to output graph.}\label{line:favor_no_edge}
%      \ENDIF
% \ENDFOR
% \RETURN $G_{\text{out}} = (V^*,E^*)$
% \end{algorithmic}
% \end{algorithm}

==> pseudocode/4_causal_expansion.tex <==
\begin{algorithm}[t]
\KwIn{a set of disjoint subsets $\{D_1...D_N\}$}
\KwResult{$\{S_1,\ldots,S_N\}$ a set of overlapping subsets}

    $S_{i} \gets D_{i} \cup \outerboundary(D_i)\;(\forall 1 \leq i \leq N)$\;
    \Return $\{S_1,\ldots,S_N\}$\;

\caption{\texttt{causal\_expansion}$(\{D_1...D_N\})$}
\label{alg:full_cd}
\end{algorithm}

% \begin{algorithm}[h]
% \caption{\texttt{causal\_expansion}$(\{D_1...D_N\})$}\label{alg:full_cd}
% \begin{algorithmic}
% \REQUIRE a set of disjoint subsets $\{D_1...D_N\}$
% \FOR{$i \in N$}
%     \STATE $S_i \gets D_i \cup \outerboundary(D_i) $
% \ENDFOR
% \ENSURE $\{S_1...S_N\}$ a set of overlapping subsets

% \end{algorithmic}
% \end{algorithm}

==> sections/mag_algorithms.tex <==
\textcolor{red} {
Notes: 
\begin{itemize}
    \item Only constraint based methods are proved to be consistent. For score based methods, the theorem that proves consistency has only been proven for DAGs but many score based methods implicitly assume it and search greedily (Hu, Evans 2024). 
    \item A method to a PAG to a MAG in the equivalence class exists for when there is no selection bias (as is our case)
\end{itemize}
Proof with MAGs: 
% TODO add definition of latent MAG 
\begin{itemize}
    \item FCI and RFCI give us the true PAG in infinite data limit. Using PAG2MAG we can get a MAG within the MEC of the latent (true) MAG. 
    \item Show that all directed information is recovered in Lemma 1, this renders bi-directed edges auxiliary
    \item Show that projected edges can still be screened using edge/no edge conflicts
    \item But now we will also get directional conflicts (loops). These are conflicts between nodes that cannot be d-separated but who's direction cannot be determined with observational data. Choose a direction based on the optimal RIC score to resolve these cycles. 
    \item Prove that this still gives us a DAG within the MEC. (1) All v\_structures are covered by the causal partition so this information is retained (2) Skeleton is recovered because all directed info is recovered and projected edges are discarded
\end{itemize}
Proof with PAGs: 
\begin{itemize}
    \item FCI, RFCI give us the true PAG in the infinite data limit 
    \item For o-o edges, this implies these nodes cannot be d-separated but that the direction cannot be determined
    \item PAG representation gives us a way to screen projected directed edges from true directed edges, so why would we need the causal partition?
    \item We need the causal partition to show that (1) the skeleton is recovered via edge coverage (2) the v\_structures are recovered in the expansive causal partition. We cannot use Lemma 1 in the same way since a PAG is not exactly defined as a projection of a DAG whereas a MAG is. Therefore it is unclear if the directed inforamtion (i.e. v\_structures will be recovered) 
\end{itemize}

\begin{table}[t]
\centering
\caption{Algorithms that operate on MAG or PAG graph class. Analysis for Assumption 1. }
\label{tab:ecoli}
\begin{tabular}{rllll}
\toprule
    Algorithm & Graph class  & Consistency? & Type 
    \\
\midrule
    GPS (Classen 2022) & PAG & No & Greedy score 
    \\
    GESMAG (Hu, Evans 2024) & MAG & No & Greedy score 
    \\
    BB (Rantaner 2021)  & MAG & No & Greedy score 
    \\
    GSMAG (Triantafillou 2016)  & MAG & No & Greedy score
    \\
    RFCI (Colombo 2012) & PAG & Yes & Constraint
    \\
    FCI (Spirtes 1999) & PAG & Yes & Constraint
    \\
\bottomrule
\end{tabular}
\end{table}

}


==> sections/problem_archived.tex <==
%%%% THIS IS AN ARCHIVED FILE
% Keeping this around in case some of these definitions are useful for future writing

\subsection{Definitions}
\begin{itemize}
    \item \textbf{Network Community} - nodes of a network are grouped into (potentially overlapping) sets of nodes such that each set of nodes is densely connected internally. Network communities shed light on the function of a system since communities often correspond to functional units of the system.  
    \item \textbf{Skeleton} - An undirected graph corresponding to all the edges in a directed acyclic graph.  
    \item \textbf{CPDAG} - Completed Partially Directed Acyclic Graph. A mixed graph (i.e., a graph with both directed and undirected edges) that represents the Markov Equivalence Class of a graph and is often the output of observational causal learners.
    \item \textbf{PDAG} - Partially Directed Acyclic Graph. A mixed graph that does not necessarily represent the Markov Equivalence class. 
    % \item \textbf{I-equivalent} - Two graphs are I-equivalent if they share the same skeleton and v-structures. 
    \item \textbf{v-structure} - A collider set $\{X,Y,Z\}$ s.t $X \rightarrow Y$ and $Z\rightarrow Y$ i.e. parent nodes share a child. 
    \item \textbf{Consistency} - An algorithm that provably finds the true graph $G^*$ in the infinite data limit.
    \item For a network $G=(V,E)$, a partition $P(G): G \to \{G_k = (V_k, E_k)\}$ s.t. $\bigcup V_k = V$ and $E_k =\{e \in E | $e connects nodes in $ V_k \}$. We will call the set $\{G_k\}$ subgraphs defined by the partition. 
    \item For a set of networks $\{G_k=(V_k,E_k)\}$, the union over the set of graphs $\bigcup{G_k} =\{V=\bigcup{V_k}, E=\bigcup{E_k}\}$ where bidirectional edges in the resultant graph are treated as undirected edges.
    \item Data is represented by a matrix $\textbf{X}=\{X_i^n\}_{i\in 1:d} \in \mathbb{R}^{n\times d}$, for $d$ random variables $X$ measured over $n$ samples. Column-wise subsets of $\textbf{X}$ are marked with a subscript: e.g. for a subset of nodes $S$, the corresponding subset of data is $\textbf{X}_{S_i}=\{X_i^n\}_{X_i \in S}$.
\end{itemize}

% \subsection{Sketch of Proof}
% We want to prove that causal learners that learn on (certain) partitions of the network are consistent. And for other partitions we want to define bounds for what will be missing in the resolved graph.  We assume the causal learner itself is consistent -- that is given infinite observational and interventional data, the learner will always find the true graph via maximization of a score function. We also assume we have the skeleton or CPDAG of the true graph, from which we can estimate the Markov Blankets. 

% \textbf{Edge cases}:
% \begin{enumerate}
%     \item If $P(G) = \{MB(X) | X \in V\}$ then in the infinite data limit, overlapping resolved subgraphs will be non-conflicting and a union over subgraphs does not lose any information.
%     \item If $G$ consists of subgraphs with no inter-subgraph edges and the partition perfectly identifies these subgraph then the union over subgraphs does not lose any information.
%      \ashka{these two edge cases need to be \enquote{mathified}}
% \end{enumerate}

% \textbf{Other cases}:
% Other partitions can break Markov Blankets and therefore we do not expect the union over subgraphs to equal the true optimal graph. Instead, we want to prove that the exclusion of nodes in the $MB(X)$ for a subgraph that includes $X$ only results in missing edges between subgraphs. That is each subgraph can be optimally learned, but the relationship between subgraphs will not be determined. Instead, we can determine those edges in a post-processing step where we learn edges between \enquote{super-nodes}.

% If $X_i \in MB(X_j) \implies X_i, X_j $ share an edge or are spouses. Spouses are defined by nodes that share a child (i.e they form a v-structure). A partition that places $X_i$ in one subgraph and $X_j$ in another subgraph as long as they are \textbf{not} spouses can be locally resolved and only miss edges between partitions. 

% Since v-structure can be determined using the PC algorithm and Meek rules this should be programmatically achievable to do. A partioning scheme based on community detection will attempt to minimize the number of edges between subgraphs and therefore will minimize the number of causally unresolved edges between subgraphs defined by the partitions. 

% \begin{assumption}
%     We have a causal learner $\mathscr{C}:\mathbb{R}^{n\times |V|} \rightarrow G$ which estimates the optimal graph from data. $\mathscr{C}$ optimizes a consistent score function $\argmax_{G} \mathit{score}(G)$. An example of a consistent score function is the Bayesian Information Criteria (BIC) (ref proof in Koller's book). 
% \end{assumption}

% \begin{assumption}
%     We have a CPDAG $S=(V,E)$ that contains the skeleton and v-structures in the true graph. Note that the PC algorithm achieves this in the infinite data limit. 
% \end{assumption}

% \begin{theorem}
%     Given $\mathscr{C}$ and $S$, we can design a consistent parallel algorithm using partitions of the skeleton $S$ according to Markov Blankets $MB(X)$ for each node $X \in V$ 
% \end{theorem}

% \begin{proof}
%     The proof is structured in three parts corresponding to a global $\rightarrow$ local $\rightarrow$ global learning algorithm: obtaining a partitioned graph from the skeleton $S$ (Lemma 4), locally learning using $\mathscr{C}$ (Lemma 5), and globally resolving subgraphs (Lemma 6).
    
% \begin{lemma}
%     We can find a set of nodes $T(X)$ s.t. $MB(X) \subseteq T(X)$ for every node $X \in V$. 
% \end{lemma}

% \begin{proof}
%     For every node $X$ in $V$, the $MB(X)$ is defined as the parents, children and parents of children. Define $T(X) = \{$ Find all neighbors of $X$ in $S$ within radius of 2 $\}$. Since $MB(X)$ consists of nodes of distance at most 2 from $X$, this implies $MB(X) \subseteq T(X)$.
% \end{proof}

% \begin{lemma}
%     Let $A={X\cup MB(X)}$ and $B={X\cup T(X)}$. $G_{A}$ is the output of the causal learner on the subset of the matrix defined by $A$: $G_{A} = \mathscr{C}(D_A)$. $G_{B}$ is output of the causal learner on the subset of the matrix defined by $B$: $G_{B} = \mathscr{C}(D_B) $. Then $G_{A} \subseteq G_{B}$
% \end{lemma}

% \begin{proof}
%      Structure argument: $G^* = \mathscr{C}(D)$. $G_{A} \subseteq G^*$ because $\mathscr{C}$ is consistent \ashka{TODO this needs to be proved}. $G_{B} \subseteq G^*$. Since $|A| \leq |B| \implies G_{A} \subseteq G_{B}$
%      \newline
%      Score argument (use the fact that the score function is decomposable): $G_{A} = \argmax_G score(G:D_A) = \argmax_G\sum_{i \in A} FamScore(X_i|Pa_{X_i}^G,D_A)$. \newline
%      $G_{B} = \argmax_G score(G:D_B) = \argmax_G\sum_{i \in B} FamScore(X_i|Pa_{X_i}^G,D_B) = \argmax_G\left(\sum_{i \in A, Pa(X_i) \in A}FamScore(X_i|Pa_{X_i}^G,D_A) + \sum_{i \in A, Pa(X_i) \notin A}FamScore(X_i|Pa_{X_i}^G,D_B) + \sum_{i \in B / A}FamScore(X_i|Pa_{X_i}^G,D_B)\right)$. \newline
%      $\argmax_G(X+Y) = \argmax_G(X)\cup\argmax_G(Y)$ \ashka{TODO prove this, under what assumptions?}
%      Decompose argmax into union, then first term is equal to $G_{A}$ therefore $ G_{A} \subseteq G_{B}$
% \end{proof}

% \begin{lemma}
%     $\mathscr{C}(S) = \bigcup_{S_k \in P(S)}\mathscr{C}(S_k)$ if $P(S)=\{T(X) | X \in V\}$
% \end{lemma}

% \begin{proof}
%      TODO need to show that $\mathscr{C}(MB(X)) \subseteq \mathscr{C}(S)$
% \end{proof}

% \end{proof}


\begin{assumption}
\label{assump:dag}
    The distribution over the random variables $X$ is induced by a DAG: $G=(V,E)$.
\end{assumption}

\begin{assumption}
We have a superstructure $C$ that constrains the true graph $G^*$. This means all edges in $G^*$ are in $C$, but not all edges in $C$ are necessarily in $G^*$. An undirected edge in $C$ constrains edges in both directions e.g an undirected edge $(i,j)$ may constrain an edge $i\rightarrow j$ or $j\rightarrow i$ in $G^*$. 
\end{assumption}

\begin{definition}
    The space of potential DAGs over a vertex set $S$ is defined by $\textbf{G}_S$ where $S \subseteq V$.
    %, the space of CPDAGs over a vertex set $S$ is defined by $\textbf{C}_S$.
\end{definition}

\begin{assumption}
    We have access to a consistent structure learning algorithm $\mathscr{A}$ that operates on data matrix $\textbf{X}_{S_i}$ for a subset of random variables $S_i \subseteq{V}$. $\mathscr{A}:\mathbb{R}^{n\times |S|} \rightarrow \textbf{G}_S$. Consistent structure learners include PC, FCI and GES for observational data \footnote{When only observational data is available, the true DAG is not identifiable. Therefore, a consistent structure learner operating on observational data estimates the Markov Equivalence Class of the true graph instead.}, and IGSP for interventional data. We additionally assume that any subset $S_i$ satisfies the assumptions needed for $\mathscr{A}$ to be consistent e.g. for PC and GES we assume causal sufficiency (no confounders). \ashka{Subsets of nodes must satisfy assumptions of the causal learning algorithm $\mathscr{A}$. For the PC and GES algorithm, this means causal faithfulness (d-separation and independence are equivalent) and causal sufficiency (no shared ancestors outside of subset). Are these necessarily needed? In the case of the latent PDAG, isn't it ok for there to be confounders since we can add an edge between to two variables? ...without this we would have to ensure that our partitioning algorithm also adheres to these assumptions which could be very restrictive }
\end{assumption}

\begin{figure}
\includegraphics[width=0.9\linewidth]{figs/LCPDAG.png}
\caption{(a) Example of latent CPDAG of $G$ when $\{X_1, X_3\} \in S$. This follows the first bullet point in \ref{def:lcpdag}. (b) Example of latent CPDAG of $G$ when $\{X_1, X_5\} \in S$. This follows the second bullet point in \ref{def:lcpdag}}
\label{fig:lcpdag}
\end{figure}
We use the following definition of a latent PDAG.
\begin{definition}[Latent PDAG]
    Let G be a DAG with variables $V$ and $S \subset V$. The latent PDAG $L(G, S)$ is the PDAG that contains all nodes in $S$, all edges between nodes in $S$ and additionally:
    \begin{itemize}
        \item a directed edge between $X, Y \in S$ if there is a directed path from $X$ to $Y$ where all intermediate nodes are in $V \setminus S$.
        \item an undirected edge between $X$, $Y$ if there is a path such that every non-endpoint is a collider in $V \setminus S$ and there are arrowheads towards $X$ and $Y$ on the adjacent edges on the path. 
    \end{itemize}
    \label{def:lcpdag}
\end{definition}

\begin{theorem}
    $\mathscr{A}(X) = \mathscr{F}(\bigcup_{S_i}\mathscr{A}(X_{S_i}))$ in the infinite data limit, where the subsets $S_i$'s form a covering set over $C$ s.t. $\bigcup_{i}C_{S_i}=C$  and $\mathscr{F}$ is a function over graph space $\mathscr{F}:G_{S} \rightarrow G_{S}$.
\end{theorem}


In other words, we can break the causal discovery problem into overlapping subproblems defined by subsets $S_i$ over the vertex set. The subsets must be defined so that each edge in $C$ is covered i.e. the union of $C_{S_i}$ is equal to $C$. We can then locally learn, merge the results by taking the union over locally resolved graphs, and apply a graph operation to achieve the same result as learning over the full vertex set. 

\begin{proof}
From Lemma 1 in \cite{faller2023self}, we know that $\mathscr{A}(X_{S_i})=L(G, S_i)$ in the infinite data limit when all $S_i$'s fulfill the assumptions of the algorithm $\mathscr{A}$. 

From the definition of $L$, a union over all subgraphs $L(G,S_i)$ may introduce new edges not present in $G$. We call this edge set the projected edge set $P_i$: $\mathscr{A}(X_{S_i}) = L(G, S_i) = G_i + P_i$ where $G_i \subset G$. This means $\bigcup_{S_i}\mathscr{A}(X_{S_i}) = \bigcup_{S_i}L(G, S_i) = G + P$ since $S_i$ is a covering set over $C$ which contains all edges in $G$. 

Now we define a function $\mathscr{F}$ as the function that removes the projected edges set $P$. First, we prove the following lemmas which will show our reasoning for how we define $\mathscr{F}$. 

\begin{definition}[Agreement]
\label{def:agreement}
    At a high level, given a pair of subgraphs, we say that the subgraphs are in agreement if the following conditions are met regarding the nodes that exist in both subgraphs:
    \begin{enumerate*}[label=\textit{(\roman*)}]
        \item an edge between two nodes exists in both subgraphs
        and
        \item direction (or lack thereof) for edges in both subgraphs are equivalent.
    \end{enumerate*}
% 
    Formally, a pair of subgraphs $\subgraph{i} = (S_i, E_i)$ and $\subgraph{j} = (S_j, E_j)$ are in agreement if $\forall u, v\in S_i \cap S_j$,
    \begin{enumerate}[label=(\roman*)]
        \item $(u,v) \in E_i \wedge (u,v) \in E_j$, or
        \item $(v,u) \in E_i \wedge (v,u) \in E_j$, or
        \item $\{u,v\} \in E_i \wedge \{u,v\} \in E_j$, or
        \item no edge containing $u$ and $v$ is in either $E_i$ or $E_j$.
    \end{enumerate}
\end{definition}

\begin{definition}[Conflict]
\label{def:conflict}
    Given some pair of subgraphs, $\subgraph{i}$ and $\subgraph{j}$, we say that a conflict arises during the union of these subgraphs when they are not in agreement (see Def.~\ref{def:agreement}).
\end{definition}


  


\begin{lemma}
    Given a consistent structure learner $\mathscr{A}$ in the infinite data limit, conflicts can only arise between `edge' and `no edge' and only in the presence of projected edges.
\end{lemma}

It is worth noting that a consistent structure learner implies $\forall u,v \in S_i$, $(u,v) \in G^* \Rightarrow (u,v) \in \mathscr{A}(S_i)$ but $(u,v) \in G^* \nRightarrow (u,v) \in \mathscr{A}(S_i)$ due to the presence of projected edges. Therefore $\forall (u,v) \in G^*$, $(u,v)$ must agree across all subgraphs.

\begin{proof}

We prove this in a case-by-case manner while considering two latent PDAGs, $\mathscr{A}(S_i) = \subgraph{i} =(S_i, E_i)$ and $\mathscr{A}(S_j) = \subgraph{j}=(S_j, E_j)$. %Without loss of generality, we will assume that 
$S_i \cup S_j = V$.
% $\bigcup{S_i, S_j} = V$.

\textsc{Case I.}
Consider the case of a directionality conflict between two subgraphs such that either of the directions is flipped, more formally,
\begin{equation}
    \left[
        (u,v) \in E_{i}
        \wedge
        (u,v) \notin E_{j}
    \right]
    \wedge 
    \left[
        (v,u) \notin E_{i}
        \wedge
        (v,u) \in E_{j}
    \right].
\end{equation}
If $(u,v) \in G^*$ then $(u,v)$ agrees across all subgraphs (see note). Otherwise if $(u,v) \notin G^*$ then it is a projected edge. Because $(u,v)$ and $(v,u)$ are directed, the projected edge is a result of the first case in \ref{def:lcpdag}. This means there is a directed path in $G^*$ where all intermediates are outside of the subset. Thus, if $(u,v) \in G_{S_i}$ and $(v,u) \in G_{S_j}$ this means there exists a path from $u$ to $v$ in $S_j$ and there exists a path from $v$ to $u$ in $S_i$. However, the presence of both paths implies a cycle in $G^*$ which contradicts Assumption \ref{assump:dag}.

\textsc{Case II.}
Consider the case of a conflict in edge type between two subgraphs such that 
\end{proof}

\begin{lemma}
    We can define a partition over variables to ensure that there are no projected edges that do not result in a conflict.
\end{lemma}
\begin{proof}
    During partition, ensure that for any subset $S_i$ with path $p$ outside of $S_i$, there is an $S_j$ that contains the adjacent nodes on the path $p$.
\end{proof}
Lemmas 1, 2 ensure that there is a projected edge if and only if there is a conflict in the union.
\begin{lemma}
     We define $\mathscr{F}$ as the function that resolves conflicts with the absence of an edge over the presence of an edge. This screens all projected edges and results in the true graph.  
\end{lemma}
\begin{proof}
    TODO
\end{proof}





A conflict occurs while merging subgraphs when overlapping nodes between subgraphs do not share the same edge set. Since each learned subgraph is a projection of the true graph $G$, conflicts only arise due to edges added as a result of one of the conditions in \ref{def:lcpdag}. Since the rest of the edges in the learned subgraphs are consistent with the true graph, any other overlapping nodes will be consistent with each other. If we can ensure that the projected set $P$ always results in a conflict between subgraphs, we can define $\mathscr{F}$ as the function that resolves these conflicts by favoring 'no edge' over 'edge' -- thereby screening out the projected set.  


To ensure the projected set $P$ always results in a conflict we need to be more specific in how we partition the superstructure and therefore how we define $S$. For any partition $S_i$, edges are only added between two nodes $(x_a, x_b)$ when either a directed path or an ancestral path exists between the nodes where all intermediates are outside of $S_i$. These added projected edges are called $M_i$. Now we create another partition $S_j$ that  includes $x_a, x_b$ and also adjacent nodes $x_{a'}, x_{b'}$ along the path. If the path is fully contained by $S_j$, then $S_j$ will not include edge $x_a, x_b$ since all intermediates in the path are observed. Therefore $\cup{S_i, S_j}$ results only in conflicts over $M_i$. However, if not all intermediates are observed between $x_{a'}, x_{b'}$ in $S_j$ then the learned projection onto $S_j$ also includes an edge between $x_{a'}, x_{b'}$. Additionally the edge between $x_a, x_b$ in $S_j$ will not exist in the learned projection onto $S_j$ because now $x_a, x_b$ do not satisfy the conditions in \ref{def:lcpdag} (there are now observed intermediates within the partition). Therefore $\cup{S_i, S_j}$ again results in conflicts over $M_i$. We can see that for any $S_i$ we can construct an $S_j$ that conflicts over the projected edge set of the learned projection onto $S_i$ by ensuring that $S_j$ contains the nodes satisfying the conditions \ref{def:lcpdag} and the pair of corresponding adjacent edges. We can use the given superstructure to determine if a pair of node satisfies these conditions and which nodes are adjacent on the path. Note that even though the superstructure does not contain all directional information we can still determine if a path exists between two nodes. By defining the partition in this way that result in conflicts over the projected edge set, we can screen all $P$'s during the merging of learned subgraphs over this partition. 

$\mathscr{F}$ is a function that takes the result of a union of graphs and any edge conflicts $e_c$ over the subgraphs and outputs a trimmed graph where any edge present in the conflict is removed from the unionized graph. $\mathscr{F}:(\textbf{G},e_c) \rightarrow \textbf{G}$. 
Then $\mathscr{F}(\bigcup_{S_i}L(G, S_i), M) = G$. Since $\mathscr{A}$ is consistent structure learner  $\mathscr{A}(X) = G$.
\end{proof}

 \ashka{ Hand wavy heuristic approximation of this since path detection is expensive: During partition if we minimize conductance then nodes corresponding to 'projected' edges (as in the two cases in \autoref{fig:lcpdag}) are on the 'edge' of the partition. If we ensure that these nodes must be in at least one other partition (together), then the projected edge will conflict across these partitions (there will be partition in which the projected edge does not exist, since the cut edges must be covered together in another partition). $\mathscr{F}$ is the function that resolves these conflicts by favoring 'no edge' over 'edge' since these conflicts are identified as projected edges. }

% Which we can also identify as edges not in $C$. Then we define $\mathscr{F}$ as the function that removes the projected set of edges such that $\mathscr{F}(\mathscr{A}(X_{S_i})) = L(G,S_i) \backslash M \subset G$. Since the projection is a subset of $G$ plus additional edges, when we remove $P$ we are left with a subset of $G$. Since $S_i$ is a covering set over $C$ and C contains all edges in $G$, this implies $\bigcup_{i}\mathscr{F}(\mathscr{A}(X_{S_i}))=G$. Finally $\mathscr{A}(X)=G$ since $\mathscr{A}$ is a consistent algorithm. This concludes the proof.  


% \nathaniel{The high-level goal of the above proof is that you can reconstruct the true graph via subgraphs given that the union of the subgraphs contain all the edges in the true graph. This proof is done to make the case for partitioning. TODO - Read this paper \cite{faller2023self}.}



==> tables/ecoli.tex <==
% \begin{table*}[t]
% \centering
% \caption{Synthetically-tuned E.coli networks. Number of samples is 1e4, fix number of partitions to 20}
% \label{tab:ecoli}
% \begin{tabular}{crlllr}
%     \toprule
%     (\#nodes, \#edges) & Algorithm & SHD & TPR & FPR & Time (s)\\
%     \midrule
%     (2332, 5691) & No Partition & 1120 & 0.804 & 6.7e-5 & 9323.329 \\
%                  & PEF & 2555 & 0.554 & 6.0e-5 & 5294.902 \\
%                  & Disjoint partition & 2554 & 0.554 & 6.0e-5 & 5363.172 \\
%                  & Edge cover partition & 2297 & 0.612 & 1.2e-4 & 607.21 \\
%                  & Expansive causal partition & 2127 & 0.631 & 6.1e-5 & 891.07 \\
%     \bottomrule
% \end{tabular}
% \end{table*}


\begin{table}[t]
\centering

{\small
\begin{tabular}{rllll}
\toprule
    Algorithm & SHD $\downarrow$ & TPR $\uparrow$ & FPR $\downarrow$ & Time (hrs) $\downarrow$
    \\
\midrule
    No Partition & \textbf{805} & \textbf{0.859} & 8.5e-5 & 11.8 
    \\
    PEF & 1,766 & 0.692 & 8.3e-5& 22.3 
    \\
    Disjoint & 3,903 & 0.479& 1.2e-4 & 23.9 
    \\
    Edge Cover & 1,791 & 0.698& 1.1e-4 & 7.1  
    \\
    Expansive Causal & 1,717 & 0.701 & \textbf{6.4e-5} & \textbf{6.9} 
    \\
\bottomrule
\end{tabular}
}

\caption{Results for a synthetically-tuned E.coli network made up of $\bm{2{,}332}$ nodes and $\bm{5{,}691}$ edges. $\bm{n=10{,}000}$. We show results only for $\mathscr{A}$ = GES, as other results are ongoing.}
\label{tab:ecoli}
% \begin{tabular}{crlllr}
%     \toprule
%     (\#nodes, \#edges) & Algorithm & SHD & TPR & FPR & Time (hrs)\\
%     \midrule
%     (2332, 5691) & No Partition & 805 & 0.859 & 8.5e-5 & 11.8 \\
%                  & PEF & 21,481 & 0.708 & 3.7e-3 & 22.3 \\
%                  & Disjoint partition & 3,903 & 0.479& 1.2e-4 & 23.9 \\
%                  & Edge cover partition & 1,791 & 0.698& 1.1e-4 & 7.1  \\
%                  & Expansive causal partition & 1,717 & 0.701 & 6.4e-5 & 6.9 \\
%     \bottomrule
% \end{tabular}
\end{table}

==> tables/experiment_defaults.tex <==
\begin{table}[]
    \centering
    {\small
    \begin{tabular}{p{0.4\linewidth}p{0.5\linewidth}}
    \toprule
        Parameter& Default Value\\
    \midrule
        Network topology   & Scale-free, $m=1, m=2$ \\
         Number of nodes ($p$) & 50 \\
         Number of communities ($k$) & 2 \\
         Number of samples ($n$) &  100,000 \\
         Frac. of extraneous edges in $G$ & 0.1 \\
         $\rho$  & 0.01  \\
         $\mathscr{A}$ & GES \\
         \texttt{disjoint\_partition} & Greedy modularity \cite{clauset2004finding}\\
    \bottomrule
    \end{tabular}
    }
    
    \caption{Default parameters for empirical studies.}
    \label{tab:defaults}
\end{table}

